Nalanda: A Socio-Technical Graph for Building Software Analytics Tools at Enterprise Scale

Software development is information-dense knowledge work that requires collaboration with other developers and awareness of artifacts such as work items, pull requests, and files. With the speed of development increasing, information overload is a challenge for people developing and maintaining these systems. Finding information and people is difficult for software engineers, especially when they work in large software systems or have just recently joined a project. In this paper, we build a large scale data platform named Nalanda platform, which contains two subsystems: 1. A large scale socio-technical graph system, named Nalanda graph system 2. A large scale recommendation system, named Nalanda index system that aims at satisfying the information needs of software developers. The Nalanda graph is an enterprise scale graph with data from 6,500 repositories, with 37,410,706 nodes and 128,745,590 edges. On top of the Nalanda graph system, we built software analytics applications including a newsfeed named MyNalanda, and based on organic growth alone, it has Daily Active Users (DAU) of 290 and Monthly Active Users (MAU) of 590. A preliminary user study shows that 74% of developers and engineering managers surveyed are favorable toward continued use of the platform for information discovery. The Nalanda index system constitutes two indices: artifact index and expert index. It uses the socio-technical graph (Nalanda graph system) to rank the results and provide better recommendations to software developers. A large scale quantitative evaluation shows that the Nalanda index system provides recommendations with an accuracy of 78% for the top three recommendations.

==> Ack.tex <==
\section{Acknowledgements}
We thank B. Ashok, Christian Bird, and Denae Ford for their support of Nalanda and their valuable feedback. We also thank the interview and survey participants for their incredible insights. 

==> Authors.tex <==
\author{Chandra Maddila}
\email{chandu.maddila@gmail.com}
\affiliation{
  \institution{Microsoft Research}
  \country{USA}
}
\author{Suhas Shanbhogue}
\email{suhas0711@gmail.com}
\affiliation{
  \institution{Microsoft Research}
  \country{India}
}
\author{Apoorva Agrawal}
\email{t-aagraw@microsoft.com}
\affiliation{
  \institution{Microsoft Research}
  \country{India}
}
\author{Thomas Zimmermann}
\email{tzimmer@microsoft.com}
\affiliation{
  \institution{Microsoft Research}
  \country{USA}
}
\author{Chetan Bansal}
\email{chetanb@microsoft.com}
\affiliation{
  \institution{Microsoft Research}
  \country{USA}
}
\author{Nicole Forsgren}
\email{niforsgr@microsoft.com}
\affiliation{
  \institution{Microsoft Research}
  \country{USA}
}
\author{Divyanshu Agrawal}
\email{divagrawal@microsoft.com}
\affiliation{
  \institution{Microsoft Research}
  \country{India}
}
\author{Kim Herzig}
\email{kimh@microsoft.com}
\affiliation{
  \institution{Microsoft}
  \country{USA}
}
\author{Arie van Deursen}
\email{Arie.vanDeursen@tudelft.nl}
\affiliation{
  \institution{Delft University of Technology}
  \country{The Netherlands}
}


==> Overview.tex <==
\section{Background (Chandra)} \label{Overview}

\arie{I think we can drop this section as the ICSE reviewers/readers will have sufficient knowledge about reviewing pull requests}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{Figures/pr-states.png}
\caption{\pr{} states}
\label{fig:StateDiagram}
\end{figure}

\subsection{Azure DevOps}
Azure DevOps \cite{AzDo} is a DevOps platform that provides GIT based VCS (version control system). Additionally, it also facilitates code review management. Azure DevOps provides an interface similar to open source tools like GitHub with a page for each \pr{}. The page contains all the information that code reviewers might need for reviewing the \pr{}, such as diff of code changes, description of the code changes and functionality for adding comments, adding/removing reviewers, etc.

Azure DevOps provides rich set of REST APIs to help with mining code review data, \pr{} data, user actions, comments on the \pr{}s, etc. We use the REST APIs extensively to mine the data and pass the recommendations back.

\subsection{Code review process}
In this section, we outline the life cycle of a \pr{} (Figure \ref{fig:StateDiagram}) and the code review process followed by most of the engineering teams at ABC Corp. The process is similar to any GIT-based software development environment. The steps involved in the code review process are listed below:

\Jiyang{Shall we add the item numbers to Figure1?}

\begin{enumerate}
    \item Developer makes changes to the code (a.k.a author) and creates a \pr{} in Azure DevOps. A \pr{} typically contains a title, description, code diff of the files changed through that \pr{}.
    \item Author makes a code review request by adding a list of reviewers that they might think appropriate to review the \pr{}.
    \item All the reviewers will receive an email notification about the code review request.
    \item Reviewers will open the \pr{} in Azure DevOps and looks at the diff view to understand the code changes happening in the \pr{}.
    \item Reviewers are expected to inspect the code changes thoroughly and add inline comments if they would like something to be changed. However, all the reviewers of the \pr{} not necessarily act on the code review request.
    \item The authors will receive an email notification for every comment added by the reviewers.
    \item When the review is completed, the reviewers will change the status of the \pr{} to one of the following: `Approved', `Rejected', `Waiting for author'.
    \item Authors will respond to the code review request by making the changes suggested by the reviewers and resolving the comments made by them. If the authors do not agree with the comments, they can resolve the review comments as `Won't fix'.
    \item The process goes on till \textit{at least} one reviewer approves it and there are no unresolved comments.
    \item The author completes the \pr{} and merges the code.
\end{enumerate}


\subsection{Reviewer recommendation tools}
In addition to the manual reviewer assignment, few teams at ABC Corp developed an automated reviewer recommendation tool, based on a simple rule: those who have reviewed or authored changes to a file in the past are qualified to review that file in the future. This is similar to the models proposed by Zanjani et al \cite{7328331} and Thongtanunam et al \cite{7081824, 10.1145/2593702.2593705}. The modified code review process when using a bot-based reviewer recommendation tool is listed below:
\begin{itemize}
    \item After step-1, the bot automatically adds reviewers.
    \item If the author is not satisfied with the reviewers added automatically by the bot, they will remove the bot-suggested reviewers and/or add their own set of reviewers.
    \item All the reviewers (added by the bot, by the authors) will get an email notification about the code review request.
    \item Reviewers, if they feel they are appropriate to review the \pr{}, will start acting on the \pr{} by leaving the code review comments.
\end{itemize}


%\subsection{Neural reviewer recommender}
%Can we do better than current system? \\
%Link prediction. \\
%Our approach.

%Training frequency, performance of training and inference.

==> Study.tex <==
\section{Information and privacy expectations} \label{UserStudy}
In this section, we describe a user study investigating perceptions of information and privacy when developer data is presented on Nalanda.  We use mixed methods (interviews and surveys) for evaluation. The study was reviewed and approved by the Microsoft Research Institutional Review Board, which is an IRB federally registered with the United States Department of Health \& Human Services. A mixed-methods approach allowed us to understand user perceptions and explain emergent patterns that may not be solely available or apparent in telemetry data, particularly one with a platform that is not yet broadly rolled out to users. We situated our user study using \codebook{} because it provided participants with concrete examples of development information that aren't typically available in a private development context without a mono repo, and that allowed us to surface questions about information sharing, information discovery and expected privacy using real data, not just imagined scenarios. In this way, these insights have a higher likelihood of extending to other applications built on Nalanda.

\subsection{Study Setup}

\subsubsection{Research Questions}
We investigated the following:
\begin{description}
\item[RQ1] What are the information needs of developers and engineering managers?
\item[RQ2] Do developers' expectations about privacy related to development-related activity at work differ when the interface changes?
\end{description}
\subsubsection{Semi-structured Interviews} Interviews were conducted to investigate information discovery and privacy, and if users might use an interface like \codebook{}.

\textbf{Participants and Protocol.}\textit{} Participants included \UseMacro{InterviewResponesDevsWord} developers and \UseMacro{InterviewResponsesManagersWord} engineering managers; \UseMacro{InterviewResponsesMaleWord} participants were men and \UseMacro{InterviewResponsesFemaleWord} were women. Semi-structured interviews were conducted remotely and ranged from 30-45 minutes. Interview topics included interest in accessing information about their own and peers' development activity, expectations surrounding privacy of development-related activity, and information overload and how they typically get information (in both in-office and work-from-home contexts). We then showed a mock-up of \codebook{} and asked for reactions including if they would like it, what information they would find useful, and where they would want to see it. If the interviewee was an engineering manager, they were also asked what information they would be interested in seeing related to their team's work. Semi-structured interviews provided flexibility in exploring topics as they emerged, and are widely used in software engineering research \cite{shrestha2020here}. To assist with record keeping and coding, interviews were recorded and automatically transcribed, and themes were noted. 

\textbf{Analysis.}\textit{} Immediately following the interviews, notes were taken by the interviewer to augment the transcription, and interviews were coded for emergent themes. Following each subsequent interview, themes were revisited to see if any codes should be combined or separated. Once no new themes emerged (i.e., theoretical saturation), we concluded our interview phase. After \UseMacro{InterviewTotalResponsesWord} interviews, themes remained consistent. Finally, we reviewed notable excerpts from all interviews and organized the themes by topic. 

\subsubsection{Surveys}
Following interviews, we conducted surveys to validate and quantify the themes that emerged. 

\textbf{Respondents.} Survey participants included full-time employees who were developers or engineering managers. While their work spanned various areas across Microsoft, all had contributed to one of the 6,500 repositories and therefore had development work that was included in Nalanda, which allowed participants to access a personalized example of \codebook{} during the survey. This allowed us to elicit preliminary reactions to the information discovery, availability, and privacy needs of developers that Nalanda graph and future applications can address. 

\textbf{Protocol.} We designed our survey based on themes that emerged during our interviews, resulting in a 19-item instrument that took a median of \UseMacro{SurveyMedianResponseTimeInMinutes} to complete. Participants were shown their \codebook{} newsfeed (with their own development activity) and given the survey. Topics included demographics, the usefulness of information included in their \codebook{} feed, information pain points, privacy concerns, and current and anticipated work location (e.g., office or work-from-home). We included items asking about the usefulness of \codebook{} information, and preferences for possible features (based on jobs-to-be-done). We asked where respondents would like to see \codebook{} integrated (if at all), and their comfort level in sharing their development activity through something like \codebook{}. The full survey instrument is available online at research.microsoft.com~\cite{maddila2021nalanda}.

\textbf{Analysis.} The survey was sent to \UseMacro{SurveyTotalParticipants} people total (\UseMacro{SurveyDevParticipants} developers and \UseMacro{SurveyManagerParticipants} engineering managers) %in the United States and India ,
with \UseMacro{SurveyTotalResponse} responses (\UseMacro{SurveyDevResponse} developers and \UseMacro{SurveyMangerResponse} engineering managers), resulting in a \UseMacro{SurveyResponseRate} response rate after considering the \UseMacro{SurveyOOFResponseRate} out of office responses. Our low response rate could be due to the summer season or because we did not offer any incentives for participation. Of those respondents, 92 (67.65\%) were developers (including software development engineers, senior software engineers, etc.), and 44 (32.35\%) were engineering managers (including software engineering managers, software engineering leads, etc.). Our respondents included five women (6.17\%), 73 men (90.12\%), one who preferred to self-describe (1.32\%), and two who preferred not to answer (2.63\%). They reported an average of 10.15 years working at Microsoft, ranging from 0.6 to 29.9 years (standard deviation of 7.13).  %Do we know if this matches msft demographics?  \tom{I think the average time working at MSR is higher than normal. We also seem to have fewer women. In technical roles, around 20% are women according to https://query.prod.cms.rt.microsoft.com/cms/api/am/binary/RE4H2f8}

\subsection{Results of the study}
For each research question, we first present findings from our semi-structured interviews, with each note as a developer (D) or an engineering manager (EM). We then present our survey results. 

\subsubsection{What are the information needs of developers and engineering managers? (RQ1)}
With increasing sources of development-related information available, there remains an open question about how they want to access and integrate information about their own development activities and the development work done by their peers, and if current platforms are adequate.

\textit{A) Interviews:} Participants expressed two themes related to information needs: integration and overload.

Information integration was echoed by many interviewees; we define this as having development-related information for self and others integrated into a single, easy-to-access interface. P1 (EM) and P2 (D) discussed easily \textit{linking} design docs and associated artifacts like pull requests. P1 (EM) discussed the usefulness of graphic summaries for their teams' development activity across time periods; this reflects consolidation via visualization. P2 (D) spoke about the usefulness of a feed that updates them about teammates' current work. The ability to see detailed information about peers' work is helpful when coordinating work, and is not readily available in many other platforms. The importance of information integration is echoed in prior studies investigating information characteristics of technical tools used to build systems \cite{forsgren2016integrated}.


P5 (D) spoke about viewing the information in different ways to deal with information overload and ensure they were not missing things: using a `Most recent' view for chronologically-ordered information, an algorithmic `Relevance' view to combine information across teams, and team-only view to further filter. This speaks to strategies they use to ensure keep up on development-related information both within and across teams they collaborate with. Similar sentiments were expressed by other interviewees.

\textit{B) Survey:} Based on themes from our interviews, we developed survey items to evaluate information integration and overload. 


We asked participants to rate how useful each feature of \codebook{} was (including development activity, the news feed, and collaborators) on a five-point Likert-type scale ranging from 1= Not at all useful to 5= Extremely useful. All items were optional; of those who took the survey, 85 answered questions about \codebook{} features (63 developers and 22 engineering managers). This allowed us to capture participant reactions to a real integrated information platform instead of a hypothetical one. Table~\ref{tab:newsfeedFeedbackwithBars} lists the accumulated percentages of "Extremely useful" (Likert=5) and "Very useful" (Likert = 4) for each feature, reported for developers and engineering managers. Not all engineering managers had activity in repositories, but their direct reports did. Here, we see that \textit{Active pull requests}\textit{} (55.6\% and 54.5\% among developers and engineering managers, respectively) and \textit{Active code review requests} (49.2\% and 45.5\% among developers and engineering managers, respectively) are the highest rated features, with \textit{User details} (27.0\% and 18.2\% among developers and engineering managers, respectively) and \textit{Related People} (23.8\% and 9.1\% among developers and engineering managers, respectively) rated the lowest. The biggest difference between developers and engineering managers is seen in the \textit{Feed} (34.9\% and 9.1\% among developers and engineering managers, respectively). These findings confirm what we heard in our interviews: developers and engineering managers have different information needs. In particular, developers find a feed of detailed development-related information useful, given it's what they do and need to keep track of every day, while engineering managers are likely more interested in team-level aggregates or trends over time. This echoes recent industry research, showing that developers favor individual metrics over team-level aggregates, which are often the focus of solutions built for managers and leaders in organizations \cite{gdp2021}.


%trying more versions for the above table
\input{Tables/NewsfeedFeedbackv1Barv1}

%\input{Tables/NewsFeedback1BarDelta}

To evaluate information overload, we asked "How challenging is it for you to currently discover and manage development activity that is relevant for you?" Among our survey respondents, 53\% indicate it is a minor concern and 47\% indicate it is a major concern. If given an opportunity to skip some information to help deal with information overload, respondents indicated `comments and replies... there are so many of these it is extremely noisy' and `I would like to see current state... on the level of work items and pull requests.' The Nalanda platform provides additional applications that can address these challenges for users.


==> Tables/NewsFeedback1BarDelta.tex <==
\pgfplotsset{width=10cm,compat=1.7}

\begin{table}[t]\centering


\small
\newlength{\myboxheightB}
\settoheight{\myboxheightB}{1234567890\%}


\def\mybarchart#1{
\resizebox {#1} {\myboxheightB} {%
\begin{tikzpicture}[]
\definecolor{clr1}{RGB}{99,99,99}
\definecolor{clr2}{RGB}{240,240,240}
\begin{axis}[
axis background/.style={fill=gray!10, draw=gray!0},%fill=gray!10, draw=gray!50
axis line style={draw=none},
tick style={draw=none},
ytick=\empty,
xtick=\empty,
ymin=0, ymax=1, %1 % this is 0.70 here, the other table is 0.60
xmin=0, xmax=1] %1
\addplot [
ybar interval=0.5, %0.5
fill=black,
draw=none,
]
coordinates {(1,1) (1,1)};%1,1 1,1
\addplot [
ybar interval=0.5,%.5
fill=black,
draw=none,
]
coordinates {(1,1) (0,1)};%
\end{axis}%
\end{tikzpicture}%
}%
}



\caption{\apoorva{\codebook survey Feedback: Devs and EMs and delta } }
\label{tab:newsfeedFeedbackwithBarsForDelta}


%\resizebox{\textwidth}{!}{%
\begin{tabular}{l|p{1.7cm}|l|l}
\toprule
Feature & \thead{Developers\\(n=63)} & \thead{Engineering\\ Managers\\(n=22)}  & \multicolumn{1}{l}{\thead{Delta\\ (n=85)}} \\
%& \thead{Delta(Developers-\\Engineering\\Managers)} \\
%\cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-6}
\midrule
Active Pull Requests (C) & 55.6\% & 54.5\% & \mybarchart{0.5pt} 1\% \\
Active Code Reviews (E) & 49.2\% & 45.5\%  & \mybarchart{1.9pt} 3.8\%  \\
%\midrule
Repositories (B) & 46.0\% & 40.9\% & \mybarchart{2.55pt} 5.1\%\\
%\midrule
Active work items (D) & 34.9\% & 31.8\% & \mybarchart{1.55pt} 3.1\%\\
Feed (F) & 34.9\% & 9.1\% & \mybarchart{12.9pt} 25.8\%\\
Biography (S) & 27\% & 18.2\% & \mybarchart{4.4pt} 8.8\%\\
People you interact (G) & 23.8\% & 9.1\% & \mybarchart{7.35pt} 14.7\%\\
\bottomrule
\end{tabular}
%}%resizebox



\end{table}

==> Tables/NewsfeedFeedbackICsvsManagers.tex <==
\begin{table}
\small
\caption{\codebook{} survey feedback}
\begin{tabular}{l|r|r|r} 
\toprule
 Feature &  \thead{Developers \\ (n=63)} & \thead{Engineering\\ Managers\\ (n=22)} & \thead{Delta\\ (Developers\\ - Engineering\\ Managers)} \\
\midrule
Active \pr{}s (C) & 55.6\% & 54.5\% & 1.0\%  \\
Active code reviews (E)  & 49.2\% & 45.5\% & 3.8\%  \\
Repositories(B) & 46.0\% & 40.9\% & 5.1\% \\
Active work items (D)  & 34.9\% & 31.8\% & 3.1\%  \\
Feed (F)  & 34.9\% & 9.1\% & 25.8\%  \\
Biography (A) & 27.0\% & 18.2\% & 8.8\%  \\
People you interact (G)  & 23.8\% & 9.1\% & 14.7\%  \\
\bottomrule
\end{tabular}
\label{tab:CodebookFeedbackICvsManagers}
\end{table}


==> Tables/NewsfeedItemOrderingResponses.tex <==
\begin{table}
\caption{\TableCaptionUserResponse{}}
 \begin{tabular}{ll} 
\toprule
Choice & \% of responses \\
\midrule
Algorithmic filtering  & \UseMacro{Chronological}  \\
Chronological ordering  & \UseMacro{Algorithmic} \\
Option to switch between both & \UseMacro{Both} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/NewsfeedPrivacyResponses.tex <==
\begin{table}
\caption{\TableCaptionUserResponse{}}
 \begin{tabular}{ll} 
\toprule
Choice & \% of responses \\
\midrule
Comfortable to share all  & \UseMacro{PrivacyAll}  \\
Comfortable to share few  & \UseMacro{PrivacyFew} \\
Not Comfortable to share any & \UseMacro{PrivacyNone} \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/TableAblations.tex <==
%%%% change the numbers from pct to decimals
% \begin{table*}[t]
% \centering
% \caption{Link prediction accuracy and MRR for various configurations of parameters}
%   \begin{tabular}{l|r|r|r|r|r|r|r|r}
%     \hline
%     \multirow{2}{*}{Config} &
%       \multicolumn{4}{c}{Accuracy} &
%       \multicolumn{4}{c}{MRR} \\
      
%     &  k = 1 & k=3 & k=5 & k=7 & k = 1 & k=3 & k=5 & k=7 \\
%     \hline
%     No words or files & 1.6\% & 7.6\% & 13.3\% & 15.6\% & 0.01 & 0.04 & 0.05 & 0.06 \\

%     Words only & 21.21\% & 29.86\% & 32.47\% & 33.88\% & 0.21 & 0.25 & 0.26 & 0.32 \\

%     %Words + Files (Tanh) & 16.02\% & 27.99\% & 29.55\% & 30.43\% & 0.16 & 0.21 & 0.22 & 0.23 \\
    
%     %Words + Files (Sigmoid) & 22.36\% & 48.39\% & 50.59\% & 53.38\% & 0.22 & 0.35 & 0.36 & 0.37 \\
    
%     Words + Files & \textbf{49.99\%} & \textbf{73.25\%} & \textbf{77.95\%} & \textbf{80.41\%} & \textbf{0.49} & \textbf{0.61} & \textbf{0.68} & \textbf{0.72} \\
%     \hline
%   \end{tabular}
%   \label{tab:AblationStudy}
% \end{table*}

\begin{table*}[t]
\centering
\caption{Link prediction accuracy and MRR for various configurations of parameters}
  \begin{tabular}{lrrrrrrrr}
    \toprule
    \multirow{2}{*}{Models} &
    \multicolumn{4}{c}{Accuracy} &
      \multicolumn{4}{c}{MRR} \\
          \cmidrule(lr){2-5}
            \cmidrule(lr){6-9}          
    &  k = 1 & k=3 & k=5 & k=7 & k = 1 & k=3 & k=5 & k=7 \\
    \hline
    (1) No words or files & 0.02 & 0.08 & 0.13 & 0.16 & 0.01 & 0.04 & 0.05 & 0.06 \\

    (2) Words only & 0.21 & 0.30 & 0.32 & 0.34 & 0.21 & 0.25 & 0.26 & 0.32 \\
    
    (3) Files only & 0.29 & 0.69 & 0.73 & 0.76 & 0.29 & 0.48 & 0.49 & 0.50 \\
    (4) Words + Files & \textbf{0.49} & \textbf{0.73} & \textbf{0.77} & \textbf{0.80} & \textbf{0.49} & \textbf{0.61} & \textbf{0.68} & \textbf{0.72} \\
    \bottomrule
  \end{tabular}
  \label{tab:AblationStudy}
\end{table*}


==> Tables/TableEmbeddingRelations.tex <==
\begin{table*}
\caption{\label{tab:Relations-used}Relations ($\mathcal{R}$) used for generating embeddings}
\begin{tabular}{cll}
\toprule
 & Relation & Semantic Description\tabularnewline
\midrule
1 & PullRequest - User & Captures the author or reviewer relationship between a pull request
and a user\tabularnewline

2 & PullRequest - File & Captures the related file modification needed for a pull request\tabularnewline

3 & PullRequest - Word & Captures the semantic description of a pull request through the words\tabularnewline

%4 & User - File & Captures the user familiarity with a code file. This relation is captured
%via the pull request\tabularnewline
%\hline 
%5 & User - Word & Captures the topical expertise of the user in terms of words. Captured
%via the pull request text\tabularnewline
%\hline 
4 & File - Word & Captures the semantic description of a file.\tabularnewline

5 & Word - Word & Captures the related words in a window of size 5 in a sentence (in
the pull request title/description)\tabularnewline
\bottomrule
\end{tabular}


\end{table*}

==> Tables/TableFalseNegatives.tex <==
\begin{table}[h]
\caption{Percentage and number of false negative \pr{}s recovered by the \nrr{} model}
 \begin{tabular}{r|r|r} 
\toprule 
Top-k & \# recovered  & recovery \% \\
\midrule
1 & \UseMacro{Top1RecoveryNum} & \UseMacro{Top1RecoveryPct}\\
3 & \UseMacro{Top3RecoveryNum} & \UseMacro{Top3RecoveryPct} \\
5 & \UseMacro{Top5RecoveryNum} & \UseMacro{Top5RecoveryPct} \\
7 & \UseMacro{Top7RecoveryNum} & \UseMacro{Top7RecoveryPct} \\
\bottomrule
\end{tabular}
\label{tab:FalseNegatives}
\end{table}


==> Tables/TableFeedbackCategory.tex <==
\begin{table*}
\caption{\TableCaptionNegativeFeedback{}}
 \begin{tabular}{llr} 
\toprule
Category & Feedback & \# of feedback (\%)\\
\midrule
\feedback{1} & This \pr{} is no longer relevant to me & \UseMacro{NumberFeedbackCategory1Combined} (\UseMacro{RateFeedbackCategory1Combined})\\
%\feedback{2} & No longer work on the project/repository/team & \UseMacro{NumberFeedback2} (\UseMacro{RateFeedback2})\\
\feedback{2} & Never participate in code review & \UseMacro{NumberFeedback3} (\UseMacro{RateFeedback3}) \\
\feedback{3} & Pull request does not need reviewer & \UseMacro{NumberFeedback4} (\UseMacro{RateFeedback4}) \\
\bottomrule
\end{tabular}
\end{table*}


% \DefMacro{NumberFeedback1}{54}
% \DefMacro{RateFeedback1}{69.23\%}  % 0.69230769
% \DefMacro{NumberFeedback2}{17}
% \DefMacro{RateFeedback2}{21.79\%}  % 0.21794872
% \DefMacro{NumberFeedback3}{5}
% \DefMacro{RateFeedback3}{6.41\%}  % 0.06410256
% \DefMacro{NumberFeedback4}{2}
% \DefMacro{RateFeedback4}{2.56\%}  % 0.02564103
% \DefMacro{NumberFeedbackTotal}{78}


==> Tables/TableLinkPrediction.tex <==
\begin{table}
\caption{Link prediction accuracy and MRR}
 \begin{tabular}{lrrrr} 
\toprule 
Metric & k = 1 & k=3 & k=5 & k=7 \\
\midrule
Accuracy & 0.50 & 0.73 & 0.78 & 0.80 \\
MRR & 0.49 & 0.61 & 0.68 & 0.72  \\
\bottomrule
\end{tabular}
\label{tab:LinkPredictionAccuracy}
\end{table}

==> Tables/TableResponseDistribution.tex <==
\begin{table}
\caption{\TableCaptionUserResponse{}}
 \begin{tabular}{ll} 
\toprule
Category & \# of responses (\%) \\
\midrule
I will review this \pr{} & \UseMacro{NumberResponseC} (\UseMacro{RateResponseC}) \\
I'd like to be added to this \pr{} & \UseMacro{NumberResponseB} (\UseMacro{RateResponseB}) \\
This \pr{} is not relevant to me & \UseMacro{NumberResponseA} (\UseMacro{RateResponseA}) \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/TableUserStudy.tex <==
\iffalse

\begin{table*}
\centering
\caption{\TableCaptionUserStudyResults{}}
 \begin{tabular}{l|c|c|c} 
\toprule
Age & \# developers & \HM Accuracy & \NRR Accuracy \\
\midrule
Young & Large & \UseMacro{YoungLargeBaselineAcc} & \textbf{\UseMacro{YoungLargeNRRAcc}}\\
Young & Medium &  \UseMacro{YoungMediumBaselineAcc} & \textbf{\UseMacro{YoungMediumNRRAcc}}\\
Young & Small &  \textbf{\UseMacro{YoungSmallBaselineAcc}} & \textbf{\UseMacro{YoungSmallNRRAcc}}\\
Mid & Large &  \UseMacro{MediumLargeBaselineAcc} & \textbf{\UseMacro{MediumLargeNRRAcc}}\\
Mid & Medium & \textbf{\UseMacro{MediumMediumBaselineAcc}} & \UseMacro{MediumMediumNRRAcc} \\
Mid & Small & \textbf{\UseMacro{MediumSmallBaselineAcc}} & \UseMacro{MediumSmallNRRAcc} \\
Old & Large & \UseMacro{OldLargeBaselineAcc} & \textbf{\UseMacro{OldLargeNRRAcc}} \\
Old & Medium & \UseMacro{OldMediumBaselineAcc} & \textbf{\UseMacro{OldMediumNRRAcc}} \\
Old & Small & \textbf{\UseMacro{YoungSmallBaselineAcc}} & \textbf{\UseMacro{YoungSmallNRRAcc}} \\
\bottomrule
\end{tabular}
\end{table*}

\fi


\begin{table}
\centering
\caption{\TableCaptionUserStudyResults{}}
 \begin{tabular}{lll} 
\toprule
Repo size (\# of developers) & RM & \NRR \\
\midrule
Large & \UseMacro{LargeBaselineAcc} & \textbf{\UseMacro{LargeNRRAcc}}\\
Medium &  \UseMacro{MediumBaselineAcc}$^{\alpha}$ & \textbf{\UseMacro{MediumNRRAcc}}$^{\alpha}$\\
Small &  \textbf{\UseMacro{SmallBaselineAcc}}$^{\beta}$ & \UseMacro{SmallNRRAcc}$^{\beta}$\\
\bottomrule
\end{tabular}
\end{table}




==> Tables/TableUserStudyStats.tex <==
% \begin{table}
% \caption{Pull request distribution across dimensions}
%  \begin{tabular}{l|l|r} 
% \toprule 
% Age of the repository & No.of developers & No.of data points \\
% \midrule
% Young & Large & 8 \\
% Young & Medium & 28 \\
% Young & Small & 8 \\
% Mid & Large & 108 \\
% Mid & Medium & 82 \\
% Mid & Small & 53 \\
% Old & Large & 104 \\
% Old & Medium & 90 \\
% Old & Small & 19 \\
% \bottomrule
% \end{tabular}
% \label{tab:StartRandomSampling}
% \end{table}

\begin{table}
\caption{Pull request distribution across dimensions}
 \begin{tabular}{l|r} 
\toprule 
Repo size (\# of developers) & \# data \\
\midrule
Large & 220 \\
Medium & 200 \\
Small & 80 \\

\bottomrule
\end{tabular}
\label{tab:StartRandomSampling}
\end{table}
